Vox2Cortex: Fast Explicit Reconstruction of Cortical Surfaces from 3D MRI Scans with Geometric Deep Neural Networks

The reconstruction of cortical surfaces from brain magnetic resonance imaging (MRI) scans is essential for quantitative analyses of cortical thickness and sulcal morphology. Although traditional and deep learning-based algorithmic pipelines exist for this purpose, they have two major drawbacks: lengthy runtimes of multiple hours (traditional) or intricate post-processing, such as mesh extraction and topology correction (deep learning-based). In this work, we address both of these issues and propose Vox2Cortex, a deep learning-based algorithm that directly yields topologically correct, three-dimensional meshes of the boundaries of the cortex. Vox2Cortex leverages convolutional and graph convolutional neural networks to deform an initial template to the densely folded geometry of the cortex represented by an input MRI scan. We show in extensive experiments on three brain MRI datasets that our meshes are as accurate as the ones reconstructed by state-of-the-art methods in the field, without the need for time- and resource-intensive post-processing. To accurately reconstruct the tightly folded cortex, we work with meshes containing about 168,000 vertices at test time, scaling deep explicit reconstruction methods to a new level.

==> latex/tables/vertex_features.tex <==
\begin{table*}[t]
	\centering
	\caption{Vertex features concatenated before each mesh-deformation stage as shown in \Cref{fig:exprecs}. For each feature vector, we provide an intuitive description of the respective information that it represents. }
	\label{tab:vertex_features}
	\begin{tabularx}{\linewidth}{@{}p{0.2\linewidth}p{0.77\linewidth}@{}}
		\toprule
		Feature vector & Encoded information\\
		\midrule
		Previous vertex features & The vertex features that were generated as output from the previous mesh deformation stage.\\
		Current coordinates & The location of the vertex in 3D space as a result of the previous mesh deformation stage.\\
		Inter-mesh neighbors & The positions of the \rough{five?} closest vertices from the respective other surface, i.e., the \rough{five?} closest vertices of the pial surface for a vertex belonging to the white-matter surface and vice versa.\\
		Surface ID & A binary encoding that indicates whether the vertex belongs to a white-matter or pial surface.\\
		Image features & Features sampled from different feature maps of the \gls{cnn} at the vertex location. Since image features are only defined for discrete voxels, we interpolate them trilinearly as done by~\cite{kong2021}. \FB{[Maybe argue why we don't use lns?]} \\
		\bottomrule
	\end{tabularx}
\end{table*}
